Quantum Attacks Targeting Nuclear Power Plants: Threat Analysis, Defense and Mitigation Strategies

Nuclear power plants face a structural lifecycle asymmetry: their 60-80 year operational lifecycles exceed the anticipated arrival of Cryptographically Relevant Quantum Computers (CRQCs), so cryptographic material harvested today becomes decryptable within the service life of the systems it protects. This paper introduces a forensics-first framework for quantum resilience that treats forensic integrity as operationally essential rather than merely evidentiary, analyzing the quantum threat landscape across the Purdue architecture (L0-L5) to show how Harvest-Now, Decrypt-Later (HNDL) campaigns enabled by Shor's algorithm can retroactively compromise cryptographic foundations and undermine forensic evidence. Through two case studies, Quantum Scar and Quantum Dawn, we model attack feasibility via a conditional-chain formulation over structured expert-judgment priors anchored to documented HNDL activity and published CRQC roadmaps, yielding success probabilities of 8-78% under current defenses, where the upper bound corresponds to high-value facilities exhibiting cryptographic monoculture. We propose a defense-in-depth migration to Post-Quantum Cryptography (PQC) integrating hybrid key exchange, code and log integrity with anti-rollback, authenticated time synchronization, and side-channel-resistant implementations aligned with ISA/IEC 62443 and NIST standards, and specify seven design-level conformance criteria for validating it; modeled residual feasibility falls to 1-8% at Security Level 4 and below 1% under full PQC migration. We further contribute six MITRE ATT&CK for ICS technique extensions (T1001-T1006) as a standardized vocabulary for quantum-enabled infrastructure attacks. Quantum threats thus extend beyond cybersecurity to system safety, operational reliability, and post-incident evidence admissibility across multi-decade nuclear asset lifecycles.

==> graphs.tex <==
 

\subsection{Performance Evaluation }





\pgfplotstableread{
 protocol key_generation_time key_encryption_time key_decryption_time
 Kyber512	0.032	0.032	0.022
HQC-128	0.108	0.145	0.232
BIKE-L1	0.369	0.073	2.232
Kyber512-90s	0.593	0.026	0.016
 SIKE/SIDH-p434	2.471	5.339	2.051
SIKE-p434	2.764	4.572	4.87
SIKE-p434-compressed	4.734	7.027	5.092
 SIKE/SIDH-p434-compressed	13.678	7.266	2.148
Classic-McEliece-348864f	169.618	0.165	0.155
Classic-McEliece-348864	345.082	0.178	0.152
}\ChartKemOne
\pgfplotstableread{
 protocol key_generation_time key_encryption_time key_decryption_time 
 SIKE-p503	3.668	5.984	6.345
 SIKE-p503-compressed	6.69	9.848	6.82
 SIKE/SIDH-p503-compressed	7.608	9.649	3.091
 SIKE/SIDH-p503	36.061	6.693	2.71
}\ChartKemTwo
\pgfplotstableread{
 protocol key_generation_time key_encryption_time key_decryption_time
Kyber768-90s	0.045	0.032	0.041
Kyber768	0.214	0.046	0.032
HQC-192	0.407	0.332	0.511
BIKE-L3	0.984	0.173	6.093
SIKE-p610	6.598	11.659	11.813
SIKE-p610-compressed	13.423	19.089	14.187
 SIKE/SIDH-p610-compressed	14.925	18.086	6.288
 SIKE/SIDH-p610	55.745	14.166	6.286
Classic-McEliece-460896f	510.955	0.253	0.26
Classic-McEliece-460896	625.816	0.25	0.255
}\ChartKemThree
\pgfplotstableread{
 protocol key_generation_time key_encryption_time key_decryption_time
Kyber1024	0.052	0.053	0.046
Kyber1024-90s	0.261	0.039	0.027
HQC-256	0.542	0.6	0.926
SIKE-p751	10.787	17	18.603
 SIKE/SIDH-p751	11.011	22.193	8.787
SIKE-p751-compressed	20.999	30.359	21.811
 SIKE/SIDH-p751-compressed	27.034	37.95	12.191
Classic-McEliece-6960119f	612.225	0.382	0.267
Classic-McEliece-6688128f	628.593	0.385	0.326
Classic-McEliece-8192128f	695.723	0.483	0.319
Classic-McEliece-6960119	803.324	0.389	0.281
Classic-McEliece-6688128	833.268	0.4	0.308
Classic-McEliece-8192128	862.543	0.482	0.306
}\ChartKemFive














 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 

 
 
\pgfplotstableread{
 protocol 	length_public_key	length_secret_key	length_ciphertext
Kyber512	800	1632	768
HQC-128	2249	2289	4481
BIKE-L1	1541	5223	1573
Kyber512-90s	800	1632	768
 SIKE/SIDH-p434	330	28	330
SIKE-p434	330	374	346
SIKE-p434-compressed	197	350	236
 SIKE/SIDH-p434-compressed	197	28	197
Classic-McEliece-348864f	261120	6452	128
Classic-McEliece-348864	261120	6452	128
}\CommKemOne 
 
 
\pgfplotstableread{
 protocol 	length_public_key	length_secret_key	length_ciphertext 
SIKE-p503	378	434	402
SIKE-p503-compressed	225	407	280
 SIKE/SIDH-p503-compressed	225	32	225
 SIKE/SIDH-p503	378	32	378
}\CommKemTwo 
 
 
\pgfplotstableread{
 protocol 	length_public_key	length_secret_key	length_ciphertext 
Kyber768-90s	1184	2400	1088
Kyber768	1184	2400	1088
HQC-192	4522	4562	9026
BIKE-L3	3083	10105	3115
SIKE-p610	462	524	486
SIKE-p610-compressed	274	491	336
 SIKE/SIDH-p610-compressed	274	39	274
 SIKE/SIDH-p610	462	39	462
Classic-McEliece-460896f	524160	13568	188
Classic-McEliece-460896	524160	13568	188
}\CommKemThree
\pgfplotstableread{
 protocol 	length_public_key	length_secret_key	length_ciphertext 
Kyber1024	1568	3168	1568
Kyber1024-90s	1568	3168	1568
HQC-256	7245	7285	14469
SIKE-p751	564	644	596
 SIKE/SIDH-p751	564	48	564
SIKE-p751-compressed	335	602	410
 SIKE/SIDH-p751-compressed	335	48	335
Classic-McEliece-6960119f	1047319	13908	226
Classic-McEliece-6688128f	1044992	13892	240
Classic-McEliece-8192128f	1357824	14080	240
Classic-McEliece-6960119	1047319	13908	226
Classic-McEliece-6688128	1044992	13892	240
Classic-McEliece-8192128	1357824	14080	240
}\CommKemFive 






\pgfplotstableread{
 protocol key_generation_time signing_time verification_time
SPHINCS+-Haraka-128f-simple	0.449	10.351	0.641
SPHINCS+-Haraka-128f-robust	0.525	12.209	0.933
SPHINCS+-SHA256-128f-simple	1.155	28.111	3.093
SPHINCS+-SHAKE256-128f-simple	1.671	41.603	4.378
SPHINCS+-SHA256-128f-robust	1.796	45.721	5.944
SPHINCS+-SHAKE256-128f-robust	2.758	69.731	8.173
Falcon-512	12.686	0.525	0.11
SPHINCS+-Haraka-128s-simple	26.299	206.082	0.276
SPHINCS+-Haraka-128s-robust	31.062	246.962	0.38
SPHINCS+-SHA256-128s-simple	66.406	497.387	1.133
SPHINCS+-SHAKE256-128s-simple	97.762	759.223	1.577
SPHINCS+-SHA256-128s-robust	106.981	822.939	2.04
SPHINCS+-SHAKE256-128s-robust	175.605	1351.929	2.897
}\ChartSigOne


\pgfplotstableread{
 protocol key_generation_time signing_time verification_time
Dilithium2-AES	0.039	0.129	0.04
$\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Dilithium2	0.495	0.179	0.073
}\ChartSigTwo

















\pgfplotstableread{
 protocol key_generation_time signing_time verification_time
Dilithium3-AES	0.053	0.136	0.056
Dilithium3	0.13	0.26	0.107
SPHINCS+-Haraka-192f-simple	0.69	18.552	0.987
SPHINCS+-Haraka-192f-robust	0.761	21.338	1.397
SPHINCS+-SHA256-192f-simple	1.562	45.656	4.596
SPHINCS+-SHAKE256-192f-simple	2.541	64.038	6.419
SPHINCS+-SHA256-192f-robust	2.918	72.277	8.944
SPHINCS+-SHAKE256-192f-robust	3.988	113.089	12.156
SPHINCS+-Haraka-192s-simple	37.208	368.562	0.387
SPHINCS+-Haraka-192s-robust	47.752	495.883	0.553
SPHINCS+-SHA256-192s-simple	95.411	945.129	1.656
SPHINCS+-SHAKE256-192s-simple	149.356	1354.498	2.251
SPHINCS+-SHA256-192s-robust	158.441	1544.76	3.466
SPHINCS+-SHAKE256-192s-robust	253.931	2280.318	4.048
}\ChartSigThree


\pgfplotstableread{
 protocol key_generation_time signing_time verification_time
Dilithium5-AES	0.083	0.165	0.082
Dilithium5	0.145	0.25	0.128
SPHINCS+-Haraka-256f-simple	1.641	35.458	0.985
SPHINCS+-Haraka-256f-robust	1.963	43.332	1.497
SPHINCS+-SHA256-256f-simple	4.203	92.525	4.788
SPHINCS+-SHAKE256-256f-simple	6.331	131.032	6.443
SPHINCS+-SHAKE256-256f-robust	10.769	225.656	12.088
SPHINCS+-SHA256-256f-robust	11.191	227.23	12.289
SPHINCS+-Haraka-256s-simple	28.888	379.874	0.567
SPHINCS+-Haraka-256s-robust	32.063	464.21	0.807
Falcon-1024	34.212	1.003	0.199
SPHINCS+-SHA256-256s-simple	60.923	753.914	2.375
SPHINCS+-SHAKE256-256s-simple	95.445	1167.943	3.274
SPHINCS+-SHAKE256-256s-robust	165.735	1978.128	5.891
SPHINCS+-SHA256-256s-robust	172.376	1978.375	6.038
}\ChartSigFive












\pgfplotstableread{
 protocol 	length_public_key	length_secret_key	length_signature
SPHINCS+-Haraka-128f-simple	32	64	17088
SPHINCS+-Haraka-128f-robust	32	64	17088
SPHINCS+-SHA256-128f-simple	32	64	17088
SPHINCS+-SHAKE256-128f-simple	32	64	17088
SPHINCS+-SHA256-128f-robust	32	64	17088
SPHINCS+-SHAKE256-128f-robust	32	64	17088
Falcon-512	897	1281	690
SPHINCS+-Haraka-128s-simple	32	64	7856
SPHINCS+-Haraka-128s-robust	32	64	7856
SPHINCS+-SHA256-128s-simple	32	64	7856
SPHINCS+-SHAKE256-128s-simple	32	64	7856
SPHINCS+-SHA256-128s-robust	32	64	7856
SPHINCS+-SHAKE256-128s-robust	32	64	7856
}\CommSigOne


\pgfplotstableread{
 protocol 	length_public_key	length_secret_key	length_signature
Dilithium2-AES	1312	2528	2420
$\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Dilithium2	1312	2528	2420
}\CommSigTwo













\pgfplotstableread{
 protocol 	length_public_key	length_secret_key	length_signature
Dilithium3-AES	1952	4000	3293
Dilithium3	1952	4000	3293
SPHINCS+-Haraka-192f-simple	48	96	35664
SPHINCS+-Haraka-192f-robust	48	96	35664
SPHINCS+-SHA256-192f-simple	48	96	35664
SPHINCS+-SHAKE256-192f-simple	48	96	35664
SPHINCS+-SHA256-192f-robust	48	96	35664
SPHINCS+-SHAKE256-192f-robust	48	96	35664
SPHINCS+-Haraka-192s-simple	48	96	16224
SPHINCS+-Haraka-192s-robust	48	96	16224
SPHINCS+-SHA256-192s-simple	48	96	16224
SPHINCS+-SHAKE256-192s-simple	48	96	16224
SPHINCS+-SHA256-192s-robust	48	96	16224
SPHINCS+-SHAKE256-192s-robust	48	96	16224
}\CommSigThree


\pgfplotstableread{
 protocol 	length_public_key	length_secret_key	length_signature
Dilithium5-AES	2592	4864	4595
Dilithium5	2592	4864	4595
SPHINCS+-Haraka-256f-simple	64	128	49856
SPHINCS+-Haraka-256f-robust	64	128	49856
SPHINCS+-SHA256-256f-simple	64	128	49856
SPHINCS+-SHAKE256-256f-simple	64	128	49856
SPHINCS+-SHAKE256-256f-robust	64	128	49856
SPHINCS+-SHA256-256f-robust	64	128	49856
SPHINCS+-Haraka-256s-simple	64	128	29792
SPHINCS+-Haraka-256s-robust	64	128	29792
Falcon-1024	1793	2305	1330
SPHINCS+-SHA256-256s-simple	64	128	29792
SPHINCS+-SHAKE256-256s-simple	64	128	29792
SPHINCS+-SHAKE256-256s-robust	64	128	29792
SPHINCS+-SHA256-256s-robust	64	128	29792
}\CommSigFive









 \begin{figure*}[!hbtp]
 
\begin{subfigure}[t]{.5\linewidth}
 \caption{Computation time for KEM/ENC level 1 (ms)}
 \centering
 \resizebox{\linewidth}{!}{

 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Kyber512, HQC-128, BIKE-L1, Kyber512-90s, SIKE/SIDH-p434, SIKE-p434, SIKE-p434-compressed, SIKE/SIDH-p434-compressed, Classic-McEliece-348864f, Classic-McEliece-348864},
 xmin=Kyber512,
 xmax=Classic-McEliece-348864,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=25,
 ymax=200,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 20)
 rectangle
 (axis cs: {[normalized] 15}, 200);
 \addplot table[x=protocol, y=key_generation_time] {\ChartKemOne};
 \addlegendentry{\scriptsize{Key Generation}}

 \addplot table[x=protocol, y=key_encryption_time] {\ChartKemOne};
 \addlegendentry{\scriptsize{Encryption}}

 \addplot table[x=protocol, y=key_decryption_time] {\ChartKemOne};
 \addlegendentry{\scriptsize{Decryption}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Kyber512, HQC-128, BIKE-L1, Kyber512-90s, SIKE/SIDH-p434, SIKE-p434, SIKE-p434-compressed, SIKE/SIDH-p434-compressed, Classic-McEliece-348864f, Classic-McEliece-348864},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=10,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=key_generation_time] {\ChartKemOne};
 \addplot table[x=protocol, y=key_encryption_time] {\ChartKemOne};
 \addplot table[x=protocol, y=key_decryption_time] {\ChartKemOne};

 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\begin{subfigure}[t]{.5\linewidth}
 \caption{Computation time for KEM/ENC level 2 (ms)}
 \centering
 \resizebox{\linewidth}{!}{


 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={SIKE-p503, SIKE-p503-compressed, SIKE/SIDH-p503-compressed, SIKE/SIDH-p503},
 xmin=SIKE-p503,
 xmax= SIKE/SIDH-p503,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=15,
 ymax=40,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 15)
 rectangle
 (axis cs: {[normalized] 15}, 40);
 \addplot table[x=protocol, y=key_generation_time] {\ChartKemTwo};
 \addlegendentry{\scriptsize{Key Generation}}

 \addplot table[x=protocol, y=key_encryption_time] {\ChartKemTwo};
 \addlegendentry{\scriptsize{Encryption}}

 \addplot table[x=protocol, y=key_decryption_time] {\ChartKemTwo};
 \addlegendentry{\scriptsize{Decryption}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={SIKE-p503,SIKE-p503-compressed, SIKE/SIDH-p503-compressed, SIKE/SIDH-p503},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=10,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=key_generation_time] {\ChartKemTwo};
 \addplot table[x=protocol, y=key_encryption_time] {\ChartKemTwo};
 \addplot table[x=protocol, y=key_decryption_time] {\ChartKemTwo};
 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\begin{subfigure}[t]{.5\linewidth}
 \caption{Computation time for KEM/ENC level 3 (ms)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Kyber768-90s, Kyber768, HQC-192, BIKE-L3, SIKE-p610, SIKE-p610-compressed, SIKE/SIDH-p610-compressed, SIKE/SIDH-p610, Classic-McEliece-460896f, Classic-McEliece-460896},
 xmin=Kyber768-90s,
 xmax=Classic-McEliece-460896,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=25,
 ymax=200,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 20)
 rectangle
 (axis cs: {[normalized] 16}, 200);
 \addplot table[x=protocol, y=key_generation_time] {\ChartKemThree};
 \addlegendentry{\scriptsize{Key Generation}}

 \addplot table[x=protocol, y=key_encryption_time] {\ChartKemThree};
 \addlegendentry{\scriptsize{Encryption}}

 \addplot table[x=protocol, y=key_decryption_time] {\ChartKemThree};
 \addlegendentry{\scriptsize{Decryption}}
 \end{scope}
 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Kyber768-90s, Kyber768, HQC-192, BIKE-L3, SIKE-p610, SIKE-p610-compressed, SIKE/SIDH-p610-compressed, SIKE/SIDH-p610, Classic-McEliece-460896f, Classic-McEliece-460896},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=20,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=key_generation_time] {\ChartKemThree};
 \addplot table[x=protocol, y=key_encryption_time] {\ChartKemThree};
 \addplot table[x=protocol, y=key_decryption_time] {\ChartKemThree};

 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\begin{subfigure}[t]{.5\linewidth}
 \caption{Computation time for KEM/ENC level 5 (ms)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Kyber1024, Kyber1024-90s, HQC-256, SIKE-p751, SIKE/SIDH-p751, SIKE-p751-compressed, SIKE/SIDH-p751-compressed, Classic-McEliece-6960119f, Classic-McEliece-6688128f, Classic-McEliece-8192128f, Classic-McEliece-6960119, Classic-McEliece-6688128, Classic-McEliece-8192128},
 xmin=Kyber1024,
 xmax=Classic-McEliece-8192128,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=600,
 ymax=900,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 600)
 rectangle
 (axis cs: {[normalized] 20}, 900);
 \addplot table[x=protocol, y=key_generation_time] {\ChartKemFive};
 \addlegendentry{\scriptsize{Key Generation}}

 \addplot table[x=protocol, y=key_encryption_time] {\ChartKemFive};
 \addlegendentry{\scriptsize{Encryption}}

 \addplot table[x=protocol, y=key_decryption_time] {\ChartKemFive};
 \addlegendentry{\scriptsize{Decryption}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Kyber1024, Kyber1024-90s, HQC-256, SIKE-p751, SIKE/SIDH-p751, SIKE-p751-compressed, SIKE/SIDH-p751-compressed, Classic-McEliece-6960119f, Classic-McEliece-6688128f, Classic-McEliece-8192128f, Classic-McEliece-6960119, Classic-McEliece-6688128, Classic-McEliece-8192128},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=40,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=key_generation_time] {\ChartKemFive};
 \addplot table[x=protocol, y=key_encryption_time] {\ChartKemFive};
 \addplot table[x=protocol, y=key_decryption_time] {\ChartKemFive};

 \end{groupplot}
 \end{tikzpicture}}
\end{subfigure}
\caption{Computation overhead comparison between all NIST $4^{th}$ round KEM/ENC candidates}
 \end{figure*}%
 
 
 
 
 
 


 \begin{figure*}[!hbtp]
 
\begin{subfigure}[t]{.5\linewidth}
 \caption{Communication overhead for KEM/ENC level 1 (byte)}
 \centering
 \resizebox{\linewidth}{!}{

 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Kyber512, HQC-128, BIKE-L1, Kyber512-90s, SIKE/SIDH-p434, SIKE-p434, SIKE-p434-compressed, SIKE/SIDH-p434-compressed, Classic-McEliece-348864f, Classic-McEliece-348864},
 xmin=Kyber512,
 xmax=Classic-McEliece-348864,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{length(byte)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=5000,
 ymax=35000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 3000)
 rectangle
 (axis cs: {[normalized] 16}, 35000);
 \addplot table[x=protocol, y=length_public_key] {\CommKemOne};
 \addlegendentry{\scriptsize{Public Key Size}}

 \addplot table[x=protocol, y=length_secret_key] {\CommKemOne};
 \addlegendentry{\scriptsize{Secret Key Size}}

 \addplot table[x=protocol, y=length_ciphertext] {\CommKemOne};
 \addlegendentry{\scriptsize{Ciphertext Size}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Kyber512, HQC-128, BIKE-L1, Kyber512-90s, SIKE/SIDH-p434, SIKE-p434, SIKE-p434-compressed, SIKE/SIDH-p434-compressed, Classic-McEliece-348864f, Classic-McEliece-348864},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=1500,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=length_public_key] {\CommKemOne};
 \addplot table[x=protocol, y=length_secret_key] {\CommKemOne};
 \addplot table[x=protocol, y=length_ciphertext] {\CommKemOne};

 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\begin{subfigure}[t]{.5\linewidth}
 \caption{Communication overhead for KEM/ENC level 2 (byte)}
 \centering
 \resizebox{\linewidth}{!}{


 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={SIKE-p503,SIKE-p503-compressed, SIKE/SIDH-p503-compressed, SIKE/SIDH-p503-compressed, SIKE/SIDH-p503},
 xmin=SIKE-p503,
 xmax= SIKE/SIDH-p503,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{length(bytes)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=1000,
 ymax=3000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 1000)
 rectangle
 (axis cs: {[normalized] 15}, 3000);
 \addplot table[x=protocol, y=length_public_key] {\CommKemTwo};
 \addlegendentry{\scriptsize{Public Key Size}}

 \addplot table[x=protocol, y=length_secret_key] {\CommKemTwo};
 \addlegendentry{\scriptsize{Secret Key Size}}

 \addplot table[x=protocol, y=length_ciphertext] {\CommKemTwo};
 \addlegendentry{\scriptsize{Ciphertext Size}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={SIKE-p503, SIKE-p503-compressed, SIKE/SIDH-p503-compressed, SIKE/SIDH-p503-compressed, SIKE/SIDH-p503},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=400,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=length_public_key] {\CommKemTwo};
 \addplot table[x=protocol, y=length_secret_key] {\CommKemTwo};
 \addplot table[x=protocol, y=length_ciphertext] {\CommKemTwo};
 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\begin{subfigure}[t]{.5\linewidth}
 \caption{Communication overhead for KEM/ENC level 3 (byte)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Kyber768-90s, Kyber768, HQC-192, BIKE-L3, SIKE-p610, SIKE-p610-compressed, SIKE/SIDH-p610-compressed, SIKE/SIDH-p610, Classic-McEliece-460896f, Classic-McEliece-460896},
 xmin=Kyber768-90s,
 xmax=Classic-McEliece-460896,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{length(bytes)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=100000,
 ymax=600000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 100000)
 rectangle
 (axis cs: {[normalized] 17}, 600000);
 \addplot table[x=protocol, y=length_public_key] {\CommKemThree};
 \addlegendentry{\scriptsize{Public Key Size}}

 \addplot table[x=protocol, y=length_secret_key] {\CommKemThree};
 \addlegendentry{\scriptsize{Secret Key Size}}

 \addplot table[x=protocol, y=length_ciphertext] {\CommKemThree};
 \addlegendentry{\scriptsize{Ciphertext Size}}
 \end{scope}
 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Kyber768-90s, Kyber768, HQC-192, BIKE-L3, SIKE-p610, SIKE-p610-compressed, SIKE/SIDH-p610-compressed, SIKE/SIDH-p610, Classic-McEliece-460896f, Classic-McEliece-460896},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=10000,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=length_public_key] {\CommKemThree};
 \addplot table[x=protocol, y=length_secret_key] {\CommKemThree};
 \addplot table[x=protocol, y=length_ciphertext] {\CommKemThree};
 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\begin{subfigure}[t]{.5\linewidth}
 \caption{Communication overhead for KEM/ENC level 5 (byte)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Kyber1024, Kyber1024-90s, HQC-256, SIKE-p751, SIKE/SIDH-p751, SIKE-p751-compressed, SIKE/SIDH-p751-compressed, Classic-McEliece-6960119f, Classic-McEliece-6688128f, Classic-McEliece-8192128f, Classic-McEliece-6960119, Classic-McEliece-6688128, Classic-McEliece-8192128},
 xmin=Kyber1024,
 xmax=Classic-McEliece-8192128,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{length(bytes)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=100000,
 ymax=2000000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 70000)
 rectangle
 (axis cs: {[normalized] 21}, 1500000);
 \addplot table[x=protocol, y=length_public_key] {\CommKemFive};
 \addlegendentry{\scriptsize{Public Key Size}}

 \addplot table[x=protocol, y=length_secret_key] {\CommKemFive};
 \addlegendentry{\scriptsize{Secret Key Size}}

 \addplot table[x=protocol, y=length_ciphertext] {\CommKemFive};
 \addlegendentry{\scriptsize{Ciphertext Size}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Kyber1024, Kyber1024-90s, HQC-256, SIKE-p751, SIKE/SIDH-p751, SIKE-p751-compressed, SIKE/SIDH-p751-compressed, Classic-McEliece-6960119f, Classic-McEliece-6688128f, Classic-McEliece-8192128f, Classic-McEliece-6960119, Classic-McEliece-6688128, Classic-McEliece-8192128},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=30000,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=length_public_key] {\CommKemFive};

 \addplot table[x=protocol, y=length_secret_key] {\CommKemFive};

 \addplot table[x=protocol, y=length_ciphertext] {\CommKemFive};

 \end{groupplot}
 \end{tikzpicture}}
\end{subfigure}
\caption{Communication overhead comparison between all NIST $4^{th}$ round KEM/ENC candidates}
 \end{figure*}%
%





















\begin{figure*}[!h]
\begin{subfigure}[t]{.5\linewidth}
 \caption{Computation time for signature level 1 (ms)}
 \centering
 \resizebox{\linewidth}{!}{

 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={SPHINCS+-Haraka-128f-simple, SPHINCS+-Haraka-128f-robust, SPHINCS+-SHA256-128f-simple, SPHINCS+-SHAKE256-128f-simple, SPHINCS+-SHA256-128f-robust, SPHINCS+-SHAKE256-128f-robust, Falcon-512, SPHINCS+-Haraka-128s-simple, SPHINCS+-Haraka-128s-robust, SPHINCS+-SHA256-128s-simple, SPHINCS+-SHAKE256-128s-simple, SPHINCS+-SHA256-128s-robust, SPHINCS+-SHAKE256-128s-robust},
 xmin=SPHINCS+-Haraka-128f-simple,
 xmax= SPHINCS+-SHAKE256-128s-robust,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=100,
 ymax=1000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 100)
 rectangle
 (axis cs: {[normalized] 20}, 1000);
 \addplot table[x=protocol, y=key_generation_time] {\ChartSigOne};
 \addlegendentry{\scriptsize{Key Generation}}

 \addplot table[x=protocol, y=signing_time] {\ChartSigOne};
 \addlegendentry{\scriptsize{Signing}}

 \addplot table[x=protocol, y=verification_time] {\ChartSigOne};
 \addlegendentry{\scriptsize{Verification}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={ SPHINCS+-Haraka-128f-simple, SPHINCS+-Haraka-128f-robust, SPHINCS+-SHA256-128f-simple, SPHINCS+-SHAKE256-128f-simple, SPHINCS+-SHA256-128f-robust, SPHINCS+-SHAKE256-128f-robust, Falcon-512, SPHINCS+-Haraka-128s-simple, SPHINCS+-Haraka-128s-robust, SPHINCS+-SHA256-128s-simple, SPHINCS+-SHAKE256-128s-simple, SPHINCS+-SHA256-128s-robust, SPHINCS+-SHAKE256-128s-robust},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=100,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=key_generation_time] {\ChartSigOne};
 \addplot table[x=protocol, y=signing_time] {\ChartSigOne};
 \addplot table[x=protocol, y=verification_time] {\ChartSigOne};

 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\begin{subfigure}[t]{.5\linewidth}
 \caption{Computation time for signature level 2 (ms)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Dilithium2-AES, $\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Dilithium2},
 xmin=Dilithium2-AES,
 xmax=$\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Dilithium2,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=0.5,
 ymax=1,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 0.5)
 rectangle
 (axis cs: {[normalized] 1}, 1);
 \addplot table[x=protocol, y=key_generation_time] {\ChartSigTwo};
 \addlegendentry{\scriptsize{Key Generation}}

 \addplot table[x=protocol, y=signing_time] {\ChartSigTwo};
 \addlegendentry{\scriptsize{Signing}}

 \addplot table[x=protocol, y=verification_time] {\ChartSigTwo};
 \addlegendentry{\scriptsize{Verification}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Dilithium2-AES, $\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Dilithium2},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=0.5,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=key_generation_time] {\ChartSigTwo};
 \addplot table[x=protocol, y=signing_time] {\ChartSigTwo};
 \addplot table[x=protocol, y=verification_time] {\ChartSigTwo};
 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
 \begin{subfigure}[t]{.5\linewidth}
 \caption{Computation time for signature level 3 (ms)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={ Dilithium3-AES, Dilithium3, SPHINCS+-Haraka-192f-simple, SPHINCS+-Haraka-192f-robust, SPHINCS+-SHA256-192f-simple, SPHINCS+-SHAKE256-192f-simple, SPHINCS+-SHA256-192f-robust, SPHINCS+-SHAKE256-192f-robust, SPHINCS+-Haraka-192s-simple, SPHINCS+-Haraka-192s-robust, SPHINCS+-SHA256-192s-simple, SPHINCS+-SHAKE256-192s-simple, SPHINCS+-SHA256-192s-robust, SPHINCS+-SHAKE256-192s-robust},
 xmin=Dilithium3-AES,
 xmax=SPHINCS+-SHAKE256-192s-robust,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=500,
 ymax=3200,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 500)
 rectangle
 (axis cs: {[normalized] 20}, 3200);
 \addplot table[x=protocol, y=key_generation_time] {\ChartSigThree};
 \addlegendentry{\scriptsize{Key Generation}}

 \addplot table[x=protocol, y=signing_time] {\ChartSigThree};
 \addlegendentry{\scriptsize{Signing}}

 \addplot table[x=protocol, y=verification_time] {\ChartSigThree};
 \addlegendentry{\scriptsize{Verification}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={ Dilithium3-AES, Dilithium3, SPHINCS+-Haraka-192f-simple, SPHINCS+-Haraka-192f-robust, SPHINCS+-SHA256-192f-simple, SPHINCS+-SHAKE256-192f-simple, SPHINCS+-SHA256-192f-robust, SPHINCS+-SHAKE256-192f-robust, SPHINCS+-Haraka-192s-simple, SPHINCS+-Haraka-192s-robust, SPHINCS+-SHA256-192s-simple, SPHINCS+-SHAKE256-192s-simple, SPHINCS+-SHA256-192s-robust, SPHINCS+-SHAKE256-192s-robust},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=300,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=key_generation_time] {\ChartSigThree};
 \addplot table[x=protocol, y=signing_time] {\ChartSigThree};
 \addplot table[x=protocol, y=verification_time] {\ChartSigThree};

 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
 \begin{subfigure}[t]{.5\linewidth}
 \caption{Computation time for signature level 5 (ms)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Dilithium5-AES, Dilithium5, SPHINCS+-Haraka-256f-simple, SPHINCS+-Haraka-256f-robust, SPHINCS+-SHA256-256f-simple, SPHINCS+-SHAKE256-256f-simple, SPHINCS+-SHAKE256-256f-robust, SPHINCS+-SHA256-256f-robust, SPHINCS+-Haraka-256s-simple, SPHINCS+-Haraka-256s-robust, Falcon-1024, SPHINCS+-SHA256-256s-simple, SPHINCS+-SHAKE256-256s-simple, SPHINCS+-SHAKE256-256s-robust, SPHINCS+-SHA256-256s-robust},
 xmin=Dilithium5-AES,
 xmax=SPHINCS+-SHA256-256s-robust,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=1000,
 ymax=10000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 400)
 rectangle
 (axis cs: {[normalized] 20}, 10000);
 \addplot table[x=protocol, y=key_generation_time] {\ChartSigFive};
 \addlegendentry{\scriptsize{Key Generation}}

 \addplot table[x=protocol, y=signing_time] {\ChartSigFive};
 \addlegendentry{\scriptsize{Signing}}

 \addplot table[x=protocol, y=verification_time] {\ChartSigFive};
 \addlegendentry{\scriptsize{Verification}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Dilithium5-AES, Dilithium5, SPHINCS+-Haraka-256f-simple, SPHINCS+-Haraka-256f-robust, SPHINCS+-SHA256-256f-simple, SPHINCS+-SHAKE256-256f-simple, SPHINCS+-SHAKE256-256f-robust, SPHINCS+-SHA256-256f-robust, SPHINCS+-Haraka-256s-simple, SPHINCS+-Haraka-256s-robust, Falcon-1024, SPHINCS+-SHA256-256s-simple, SPHINCS+-SHAKE256-256s-simple, SPHINCS+-SHAKE256-256s-robust, SPHINCS+-SHA256-256s-robust},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=250,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=key_generation_time] {\ChartSigFive};
 \addplot table[x=protocol, y=signing_time] {\ChartSigFive};
 \addplot table[x=protocol, y=verification_time] {\ChartSigFive};

 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\caption{Computation overhead comparison between all NIST $4^{th}$ round signature candidates}
 \end{figure*}%
%














\begin{figure*}[!h]
\begin{subfigure}[t]{.5\linewidth}
 \caption{Communication overhead for signature level 1 (ms)}
 \centering
 \resizebox{\linewidth}{!}{

 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={SPHINCS+-Haraka-128f-simple, SPHINCS+-Haraka-128f-robust, SPHINCS+-SHA256-128f-simple, SPHINCS+-SHAKE256-128f-simple, SPHINCS+-SHA256-128f-robust, SPHINCS+-SHAKE256-128f-robust, Falcon-512, SPHINCS+-Haraka-128s-simple, SPHINCS+-Haraka-128s-robust, SPHINCS+-SHA256-128s-simple, SPHINCS+-SHAKE256-128s-simple, SPHINCS+-SHA256-128s-robust, SPHINCS+-SHAKE256-128s-robust},
 xmin=SPHINCS+-Haraka-128f-simple,
 xmax=SPHINCS+-SHAKE256-128s-robust,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{length(byte)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=6000,
 ymax=170000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 3000)
 rectangle
 (axis cs: {[normalized] 20}, 170000);
 \addplot table[x=protocol, y=length_public_key] {\CommSigOne};
 \addlegendentry{\scriptsize{Public Key Size}}

 \addplot table[x=protocol, y=length_secret_key] {\CommSigOne};
 \addlegendentry{\scriptsize{Secret Key Size}}

 \addplot table[x=protocol, y=length_signature] {\CommSigOne};
 \addlegendentry{\scriptsize{Signature Size}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={ SPHINCS+-Haraka-128f-simple, SPHINCS+-Haraka-128f-robust, SPHINCS+-SHA256-128f-simple, SPHINCS+-SHAKE256-128f-simple, SPHINCS+-SHA256-128f-robust, SPHINCS+-SHAKE256-128f-robust, Falcon-512, SPHINCS+-Haraka-128s-simple, SPHINCS+-Haraka-128s-robust, SPHINCS+-SHA256-128s-simple, SPHINCS+-SHAKE256-128s-simple, SPHINCS+-SHA256-128s-robust, SPHINCS+-SHAKE256-128s-robust},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=1000,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=length_public_key] {\CommSigOne};

 \addplot table[x=protocol, y=length_secret_key] {\CommSigOne};

 \addplot table[x=protocol, y=length_signature] {\CommSigOne};
 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\begin{subfigure}[t]{.5\linewidth}
 \caption{Communication overhead for signature level 2 (ms)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Dilithium2-AES, $\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Dilithium2},
 xmin=Dilithium2-AES,
 xmax=$\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Dilithium2,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{length(byte)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=1700,
 ymax=4000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 1700)
 rectangle
 (axis cs: {[normalized] 2}, 4000);
 \addplot table[x=protocol, y=length_public_key] {\CommSigTwo};
 \addlegendentry{\scriptsize{Public Key Size}}

 \addplot table[x=protocol, y=length_secret_key] {\CommSigTwo};
 \addlegendentry{\scriptsize{Secret Key Size}}

 \addplot table[x=protocol, y=length_signature] {\CommSigTwo};
 \addlegendentry{\scriptsize{Signature Size}}
 \end{scope}
 
 
 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Dilithium2-AES, $\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Dilithium2},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=1500,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 
 \addplot table[x=protocol, y=length_public_key] {\CommSigTwo};

 \addplot table[x=protocol, y=length_secret_key] {\CommSigTwo};

 \addplot table[x=protocol, y=length_signature] {\CommSigTwo};
 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
 \begin{subfigure}[t]{.5\linewidth}
 \caption{Communication overhead for signature level 3 (ms)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={ Dilithium3-AES, Dilithium3, SPHINCS+-Haraka-192f-simple, SPHINCS+-Haraka-192f-robust, SPHINCS+-SHA256-192f-simple, SPHINCS+-SHAKE256-192f-simple, SPHINCS+-SHA256-192f-robust, SPHINCS+-SHAKE256-192f-robust, SPHINCS+-Haraka-192s-simple, SPHINCS+-Haraka-192s-robust, SPHINCS+-SHA256-192s-simple, SPHINCS+-SHAKE256-192s-simple, SPHINCS+-SHA256-192s-robust, SPHINCS+-SHAKE256-192s-robust},
 xmin=Dilithium3-AES,
 xmax=SPHINCS+-SHAKE256-192s-robust,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=5000,
 ymax=50000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 5000)
 rectangle
 (axis cs: {[normalized] 23}, 50000);
 \addplot table[x=protocol, y=length_public_key] {\CommSigThree};
 \addlegendentry{\scriptsize{Public Key Size}}

 \addplot table[x=protocol, y=length_secret_key] {\CommSigThree};
 \addlegendentry{\scriptsize{Secret Key Size}}

 \addplot table[x=protocol, y=length_signature] {\CommSigThree};
 \addlegendentry{\scriptsize{Signature Size}}
 \end{scope}

 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={ Dilithium3-AES, Dilithium3, SPHINCS+-Haraka-192f-simple, SPHINCS+-Haraka-192f-robust, SPHINCS+-SHA256-192f-simple, SPHINCS+-SHAKE256-192f-simple, SPHINCS+-SHA256-192f-robust, SPHINCS+-SHAKE256-192f-robust, SPHINCS+-Haraka-192s-simple, SPHINCS+-Haraka-192s-robust, SPHINCS+-SHA256-192s-simple, SPHINCS+-SHAKE256-192s-simple, SPHINCS+-SHA256-192s-robust, SPHINCS+-SHAKE256-192s-robust},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=5000,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=length_public_key] {\CommSigThree};

 \addplot table[x=protocol, y=length_secret_key] {\CommSigThree};

 \addplot table[x=protocol, y=length_signature] {\CommSigThree};

 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
 \begin{subfigure}[t]{.5\linewidth}
 \caption{Communication overhead for signature level 5 (ms)}
 \centering
 \resizebox{\linewidth}{!}{
 \begin{tikzpicture}
 \begin{groupplot}[
 group style={
 group size=1 by 2,
 % The two plots will touch one another vertically
 vertical sep=0pt
 },
 % Common settings
 ybar,
 symbolic x coords={Dilithium5-AES, Dilithium5, SPHINCS+-Haraka-256f-simple, SPHINCS+-Haraka-256f-robust, SPHINCS+-SHA256-256f-simple, SPHINCS+-SHAKE256-256f-simple, SPHINCS+-SHAKE256-256f-robust, SPHINCS+-SHA256-256f-robust, SPHINCS+-Haraka-256s-simple, SPHINCS+-Haraka-256s-robust, Falcon-1024, SPHINCS+-SHA256-256s-simple, SPHINCS+-SHAKE256-256s-simple, SPHINCS+-SHAKE256-256s-robust, SPHINCS+-SHA256-256s-robust},
 xmin=Dilithium5-AES,
 xmax=SPHINCS+-SHA256-256s-robust,
 scaled ticks=false,
 enlarge x limits=true,
 ]
 \nextgroupplot[
 ybar,
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 legend pos=north west,
 legend cell align=left,
 ylabel={\scriptsize{time(ms)}},
 xtick=\empty,
 axis x line*=top,
 axis y discontinuity=parallel,
 ymin=5000,
 ymax=50000,
 enlarge y limits=true
 ]

 \begin{scope}
 \clip
 (axis cs: {[normalized]-1}, 5000)
 rectangle
 (axis cs: {[normalized] 23}, 50000);
 \addplot table[x=protocol, y=length_public_key] {\CommSigFive};
 \addlegendentry{\scriptsize{Public Key Size}}

 \addplot table[x=protocol, y=length_secret_key] {\CommSigFive};
 \addlegendentry{\scriptsize{Secret Key Size}}

 \addplot table[x=protocol, y=length_signature] {\CommSigFive};
 \addlegendentry{\scriptsize{Signature Size}}
 \end{scope}


 \nextgroupplot[
 bar width=1.5pt,
 width=\textwidth,
 height=.5\textwidth,
 xticklabels={Dilithium5-AES, Dilithium5, SPHINCS+-Haraka-256f-simple, SPHINCS+-Haraka-256f-robust, SPHINCS+-SHA256-256f-simple, SPHINCS+-SHAKE256-256f-simple, SPHINCS+-SHAKE256-256f-robust, SPHINCS+-SHA256-256f-robust, SPHINCS+-Haraka-256s-simple, SPHINCS+-Haraka-256s-robust, Falcon-1024, SPHINCS+-SHA256-256s-simple, SPHINCS+-SHAKE256-256s-simple, SPHINCS+-SHAKE256-256s-robust, SPHINCS+-SHA256-256s-robust},
 x tick label style={font=\scriptsize,
 rotate=45, anchor=east},
 xtick=data,
 ymin=0,
 ymax=5000,
 enlarge y limits=true,
 axis x line*=bottom
 ]
 \addplot table[x=protocol, y=length_public_key] {\CommSigFive};

 \addplot table[x=protocol, y=length_secret_key] {\CommSigFive};

 \addplot table[x=protocol, y=length_signature] {\CommSigFive};

 \end{groupplot}
 \end{tikzpicture}}
 \end{subfigure}%
 \hfill
\caption{Communication overhead comparison between all NIST $4^{th}$ round signature candidates}
 \end{figure*}%
%


